Predicting Chaotic Systems with Quantum Echo-state Networks

Recent advancements in artificial neural networks have enabled impressive tasks on classical computers, but they demand significant computational resources. While quantum computing offers potential beyond classical systems, the advantages of quantum neural networks (QNNs) remain largely unexplored. In this work, we present and examine a quantum circuit (QC) that implements and aims to improve upon the classical echo-state network (ESN), a type of reservoir-based recurrent neural networks (RNNs), using quantum computers. Typically, ESNs consist of an extremely large reservoir that learns high-dimensional embeddings, enabling prediction of complex system trajectories. Quantum echo-state networks (QESNs) aim to reduce this need for prohibitively large reservoirs by leveraging the unique capabilities of quantum computers, potentially allowing for more efficient and higher performing time-series prediction algorithms. The proposed QESN can be implemented on any digital quantum computer implementing a universal gate set, and does not require any sort of stopping or re-initialization of the circuit, allowing continuous evolution of the quantum state over long time horizons. We conducted simulated QC experiments on the chaotic Lorenz system, both with noisy and noiseless models, to demonstrate the circuit's performance and its potential for execution on noisy intermediate-scale quantum (NISQ) computers.

==> Acronyms.tex <==
%
\newacronym{ANN}{ANN}{Artificial Neural Network}
\newacronym{DNN}{DNN}{Deep Neural Network}
\newacronym{ODE}{ODE}{Ordinary Differential Equation}
\newacronym{SPDE}{SPDE}{Stochastic Partial Differential Equation}
\newacronym{FNN}{FNN}{Feed-forward Neural Network}
\newacronym{CNN}{CNN}{Convolutional Neural Network}
\newacronym{DP}{DP}{Dynamic Programming}
\newacronym{LSTM}{LSTM}{Long-Short Term Memory}
\newacronym{FC}{FC}{Fully Connected}
\newacronym{DDP}{DDP}{Differential Dynamic Programming}
\newacronym{HJB}{HJB}{Hamilton-Jacobi-Bellman}
\newacronym{PDE}{PDE}{Partial Differential Equation}
\newacronym{PI}{PI}{Path Integral}
\makeglossaries
\newacronym{NN}{NN}{Neural Network}
\newacronym{SOC}{SOC}{Stochastic Optimal Control}
\newacronym{RL}{RL}{Reinforcement Learning}
\newacronym{MPC}{MPC}{Model Predictive Control}
\newacronym{IL}{IL}{Imitation Learning}
\newacronym{RNN}{RNN}{Recurrent Neural Network}
\newacronym{DL}{DL}{Deep Learning}
\newacronym{SGD}{SGD}{Stochastic Gradient Descent}
\newacronym{SDE}{SDE}{Stochastic Differential Equation}
\newacronym{VRL}{VRL}{Variational Reinforcement Learning}
\newacronym{IDVRL}{IDVRL}{Infinite Dimensional Variational Reinforcement Learning}
\newacronym{ROM}{ROM}{Reduced Order Model}
\newacronym{ADPL}{ADPL}{Actuator Design and Policy Learning}
\newacronym{FBSDE}{FBSDE}{Forward-Backward Stochastic Differential Equation}
\newacronym{KL}{KL}{Kullback-Leibler}
\newacronym{DOF}{DOF}{Degrees of Freedom}
% \newacronym{PMP}{PMP}{Pontryagin Maximum Principle}
\newacronym{GRAPE}{GRAPE}{Gradient Ascent Pulse Engineering}
\newacronym{QND}{QND}{Quantum Non-Demolition}
\newacronym{MHD}{MHD}{magnetohydrodynamics}
\newacronym{STSO}{STSO}{Spatio-Temporal Stochastic Optimization}
\newacronym{LQR}{LQR}{Linear Quadratic Regulator}
\newacronym{STDDP}{STDDP}{Spatio-Temporal DDP}
\newacronym{RDE}{RDE}{Riccati Differential Equation}
\newacronym{1D}{1D}{1-dimensional}
\newacronym{2D}{2D}{2-dimensional}
\newacronym{3D}{3D}{3-dimensional}
\newacronym{RN}{RN}{Radon-Nikodym}
\newacronym{SNN}{SNN}{Sparse Neural Network}
\newacronym{FLOP}{FLOP}{Floating Point Operation}
\newacronym{GASS}{GASS}{Gradient-based Adaptive Stochastic Search}
\newacronym{NODE}{NODE}{Neural Ordinary Differential Equation}
\newacronym{QGASS}{QGASS}{Quantum Gradient-based Adaptive Stochastic Search}
\newacronym{MPPI}{MPPI}{Model Predictive Path Integral}
\newacronym{QVO-SS}{QVO-SS}{Quantum Variational Optimization - Single Shot}
\newacronym{QVO-MPC}{QVO-MPC}{Quantum Variational Optimization - MPC}
\newacronym{QSTSO}{QSTSO}{Quantum Spatio-Temporal Stochastic Optimization}
\newacronym{SME}{SME}{Stochastic Master Equation}
\newacronym{QRL}{QRL}{Quantum Reinforcement Learning}
\newacronym{ITC}{ITC}{Information Theoretic Control}
\newacronym{CFD}{CFD}{Computational Fluid Dynamics}
\newacronym{NP}{NP}{Non-Polynomial-Time}
\newacronym{ReLU}{ReLU}{Rectified Linear Unit}
\newacronym{NCOM}{NCOM}{Navy Coastal Ocean Model}
\newacronym{UUV}{UUV}{Unmanned Underwater Vehicle}
\newacronym{USV}{USV}{Unmanned Surface Vehicle}


% \makeListOfAcronyms





